The planar $3$-colorable subgroup $\mathcal{E}$ of Thompson's group $F$ and its even part

We study the planar $3$-colorable subgroup $\mathcal{E}$ of Thompson's group $F$ and its even part $\mathcal{E}_{\rm EVEN}$. The latter is obtained by cutting $\mathcal{E}$ with a finite index subgroup of $F$ isomorphic to $F$, namely the rectangular subgroup $K_{(2,2)}$. We show that the even part $\mathcal{E}_{\rm EVEN}$ of the planar $3$-colorable subgroup admits a description in terms of stabilisers of suitable subsets of dyadic rationals. As a consequence $\mathcal{E}_{\rm EVEN}$ is closed in the sense of Golan and Sapir. We then study three quasi-regular representations associated with $\mathcal{E}_{\rm EVEN}$: two are shown to be irreducible and one to be reducible.

==> bib.tex <==

%\begin{bibdiv}
\begin{biblist}

%\bib{ABLS}{article}{
%author={Afsar, Zahra},
%author={Brownlowe, Nathan},
%author={Larsen, Nadia S.},
%author={Stammeier, Nicolai},
%title={Equilibrium states on right LCM semigroup $C^*$-algebras},
%journal={Int. Math. Res. Not.},
%year={2017 (advance article)},
%doi={\href{https://doi.org/10.1093/imrn/rnx162}{10.1093/imrn/rnx162}},
%%note={preprint, \href{https://arxiv.org/abs/1611.01052}{arxiv:1611.01052}},
%}


\bib{A}{article}{
  AUTHOR = {Aiello, Valeriano},
     TITLE = {On the {A}lexander theorem for the oriented Thompson group
              {$\vec{F}$}},
   JOURNAL = {Algebr. Geom. Topol.},
  FJOURNAL = {Algebraic \& Geometric Topology},
    VOLUME = {20},
      YEAR = {2020},
    NUMBER = {1},
     PAGES = {429--438},
      ISSN = {1472-2747},
   MRCLASS = {57K10},
  MRNUMBER = {4071378},
MRREVIEWER = {Masakazu Teragaito},
       DOI = {10.2140/agt.2020.20.429},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.2140/agt.2020.20.429},
}

\bib{A2}{article}{ 
  title={An introduction to Thompson knot theory and to Jones subgroups},
  author={Aiello, Valeriano},
  journal={J. Knot Theory Ramifications, preprint arXiv:2211.15461},
  year={2022}
}



\bib{AB1}{article}{
author={Aiello, Valeriano},
author={Baader, Sebastian},
title={Positive oriented Thompson links},
note={accepted for publication in Communications in Analysis and Geometry, preprint \href{http://arxiv.org/abs/2101.04534}{arXiv:2101.04534}},
year={2021},
}


\bib{AB2}{article}{
  title={Arborescence of positive Thompson links},
author={Aiello, Valeriano},
author={Baader, Sebastian}, 
 note={preprint \href{http://arxiv.org/abs/2106.13648}{arXiv:2106.13648}},
journal={Pacific Journal of Mathematics},
volume={316} 
issue={2}, 
pages={237-248}, 
 year={2022}
}



\bib{ABC}{article}{
author={Aiello, Valeriano},
author={Brothier, Arnaud},
author={Conti, Roberto},
title={Jones representations of Thompson's group $F$ arising from Temperley-Lieb-Jones algebras},
journal={Int. Math. Res. Not.},
    VOLUME = {15},
    PAGES = {11209-11245},
    year={2021},
    doi={https://doi.org/10.1093/imrn/rnz240},
note={preprint \href{http://arxiv.org/abs/1901.10597}{arXiv:1901.10597}},
%year={2016},
}
%Int. Math. Res. Not. 15 (2021), 11209–11245, doi: 10.1093/imrn/rnz240 
		

\bib{AiCo1}{article}{
author={Aiello, Valeriano},
author={Conti, Roberto},
     TITLE = {Graph polynomials and link invariants as positive type
              functions on {T}hompson's group {$F$}},
   JOURNAL = {J. Knot Theory Ramifications},
  FJOURNAL = {Journal of Knot Theory and its Ramifications},
    VOLUME = {28},
      YEAR = {2019},
    NUMBER = {2},
     PAGES = {1950006, 17},
      ISSN = {0218-2165},
   MRCLASS = {43A35 (05C31 57M27)},
  MRNUMBER = {3924840},
MRREVIEWER = {Markus Neuhauser},
       DOI = {10.1142/S0218216519500068},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1142/S0218216519500068},
}


\bib{AiCo2}{article}{
author={Aiello, Valeriano},
author={Conti, Roberto},
     TITLE = {The Jones polynomial and functions of positive type on the
              oriented Jones-Thompson groups {$\vec {F}$} and {$\vec
              {T}$}},
   JOURNAL = {Complex Anal. Oper. Theory},
  FJOURNAL = {Complex Analysis and Operator Theory},
    VOLUME = {13},
      YEAR = {2019},
    NUMBER = {7},
     PAGES = {3127--3149},
      ISSN = {1661-8254},
   MRCLASS = {57M27 (05C31 43A35)},
  MRNUMBER = {4020028},
       DOI = {10.1007/s11785-018-0866-6},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1007/s11785-018-0866-6},
}		

\bib{ACJ}{article}{
author={Aiello, Valeriano},
author={Conti, Roberto},
    AUTHOR = {Jones, Vaughan F. R.},
     TITLE = {The Homflypt polynomial and the oriented Thompson group},
   JOURNAL = {Quantum Topol.},
  FJOURNAL = {Quantum Topology},
    VOLUME = {9},
      YEAR = {2018},
    NUMBER = {3},
     PAGES = {461--472},
      ISSN = {1663-487X},
   MRCLASS = {57M27 (20F65)},
  MRNUMBER = {3827807},
MRREVIEWER = {Bruno P. Zimmermann},
       DOI = {10.4171/QT/112},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.4171/QT/112},
}
		






\bib{AJ}{article}{
    AUTHOR = {Aiello, Valeriano}, % and Jones, Vaughan F. R.},
    AUTHOR = {Jones, Vaughan F. R.},
     TITLE = {On spectral measures for certain unitary representations of
              {R}. {T}hompson's group {F}},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {280},
      YEAR = {2021},
    NUMBER = {1},
     PAGES = {108777, 27},
      ISSN = {0022-1236},
   MRCLASS = {22D10 (18M30 20F65 46L37)},
  MRNUMBER = {4156130},
       DOI = {10.1016/j.jfa.2020.108777},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1016/j.jfa.2020.108777},
}
 
 \bib{TV}{article}{
author={Aiello, Valeriano},
author={Nagnibeda, Tatiana},
title={On the oriented Thompson subgroup $\vec{F}_3$ and its relatives in higher Brown-Thompson groups},
journal={Journal of Algebra and its Applications},
 volume={21}, 
 number={07}, 
note={2250139, preprint \href{http://arxiv.org/abs/1912.04730}{arXiv:1912.04730}},
year={2022},
}


 \bib{TV2}{article}{
author={Aiello, Valeriano},
author={Nagnibeda, Tatiana},
title={On the 3-colorable subgroup $\mathcal{F}$ and maximal subgroups of Thompson’s group $F$},
journal={Annales l'Institut Fourier},
  volume={73},
  number={2},
  pages={783--828},
  year={2023},
note={preprint \href{http://arxiv.org/abs/2103.07885}{arXiv:2103.07885}},
} 
  
  \bib{AP}{article}{ 
  title={Representations of Higman-Thompson groups from Cuntz algebras},
  author={Ara{\'u}jo, Francisco},
  author={Pinto, Paulo R.},
  title={Representations of Higman-Thompson groups from Cuntz algebras},
  journal={Journal of Mathematical Analysis and Applications},
volume = {509},
number = {2},
pages = {125970},
year = {2022},
  publisher={Elsevier}
%  note={preprint \href{http://arxiv.org/abs/2011.13679}{arXiv:2011.13679}},
%  journal={preprint arXiv:2011.13679},
  %year={2020}
}

 
 \bib{BP}{article}{ 
  title={Representations of Thompson groups from Cuntz algebras},
  author={Barata, Miguel},
    author={Pinto, Paulo R.},
  journal={Journal of Mathematical Analysis and Applications},
volume = {478},
number = {1},
pages = {212-228},
year = {2019},%doi = {https://doi.org/10.1016/j.jmaa.2021.125970},
  publisher={Elsevier}
}

 
 
 \bib{B}{article}{
  title={Thompson's group F},
  author={Belk, James},
    note={preprint \href{http://arxiv.org/abs/0708.3609}{arXiv:0708.3609}},
%  journal={preprint arXiv:0708.3609},
  year={2007}
}

  \bib{BM}{article}{
     AUTHOR = {Belk, James},
     AUTHOR = {Matucci, Francesco},
     TITLE = {Conjugacy and dynamics in Thompson's groups},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {169},
      YEAR = {2014},
     PAGES = {239--261},
      ISSN = {0046-5755},
   MRCLASS = {20F65},
  MRNUMBER = {3175247},
MRREVIEWER = {Dmytro M. Savchuk},
       DOI = {10.1007/s10711-013-9853-2},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1007/s10711-013-9853-2},
}
 
  
 \bib{BW}{article}{
  author={Bleak, Collin},
    author={Wassink, Bronlyn},
title={Finite index subgroups of R. Thompson's group F},
 note={preprint \href{http://arxiv.org/abs/0711.1014}{arXiv:0711.1014}},
year={2007},
}
 
 
 
 \bib{BJ}{article}{
    AUTHOR = {Brothier, Arnaud},
    AUTHOR = {Jones, Vaughan F. R.},
     TITLE = {Pythagorean representations of Thompson's groups},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {277},
      YEAR = {2019},
    NUMBER = {7},
     PAGES = {2442--2469},
      ISSN = {0022-1236},
   MRCLASS = {22D25 (20F65 46L05)},
  MRNUMBER = {3989149},
MRREVIEWER = {Bachir Bekka},
       DOI = {10.1016/j.jfa.2019.02.009},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1016/j.jfa.2019.02.009},
}
		
 
 \bib{BJ2}{article}{
    AUTHOR = {Brothier, Arnaud},
    AUTHOR = {Jones, Vaughan F. R.},
  title={On the Haagerup and Kazhdan properties of R. Thompson’s groups},
  journal={Journal of Group Theory},
  volume={22},
  number={5},
  pages={795--807},
  year={2019}
}


 \bib{BrWi}{article}{
  title={Jones' representations of R. Thompson's groups not induced by finite-dimensional ones},
  author={Brothier, Arnaud},
  author={Wijesena, Dilshan},
  journal={preprint arXiv:2211.08555},
  year={2022}
}


 \bib{Brown}{article}{
    AUTHOR = {Brown, Kenneth S.},
     TITLE = {Finiteness properties of groups},
 BOOKTITLE = {Proceedings of the {N}orthwestern conference on cohomology of
              groups ({E}vanston, {I}ll., 1985)},
   JOURNAL = {J. Pure Appl. Algebra},
  FJOURNAL = {Journal of Pure and Applied Algebra},
    VOLUME = {44},
      YEAR = {1987},
    NUMBER = {1-3},
     PAGES = {45--75},
      ISSN = {0022-4049},
   MRCLASS = {20J05 (11F75 20F05 22E40)},
  MRNUMBER = {885095},
MRREVIEWER = {Ralph Strebel},
       DOI = {10.1016/0022-4049(87)90015-6},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1016/0022-4049(87)90015-6},
}

\bib{BCS}{article}{
  title={Metrics and embeddings of generalizations of Thompson’s group F},
  author={Burillo, Jos{\'e}},
  author={Cleary, Sean},
  author={Stein, Melanie},
  journal={Transactions of the American Mathematical Society},
  volume={353},
  number={4},
  pages={1677--1689},
  year={2001}
}

 \bib{CFP}{article}{
  author={Cannon, James W.},
    author={Floyd, William J.},  
      author={Parry, Walter R.},
     TITLE = {Introductory notes on Richard Thompson's groups},
   JOURNAL = {Enseign. Math. (2)},
  FJOURNAL = {L'Enseignement Math\'{e}matique. Revue Internationale. 2e S\'{e}rie},
    VOLUME = {42},
      YEAR = {1996},
    NUMBER = {3-4},
     PAGES = {215--256},
      ISSN = {0013-8584},
   MRCLASS = {20F32 (57M07)},
  MRNUMBER = {1426438},
MRREVIEWER = {Michael L. Mihalik},
}

\bib{Cuntz}{article}{ 
  title={Simple C$^*$-algebra generated by isometries},
  author={Cuntz, Joachim},
  journal={Communications in mathematical physics},
  volume={57},
  number={2},
  pages={173--185},
  year={1977},
  publisher={Springer}
}

 \bib{DM}{article}{
    AUTHOR = {Dudko, Artem},
    AUTHOR = {Medynets, Konstantin},
     TITLE = {Finite factor representations of Higman-Thompson groups},
   JOURNAL = {Groups Geom. Dyn.},
  FJOURNAL = {Groups, Geometry, and Dynamics},
    VOLUME = {8},
      YEAR = {2014},
    NUMBER = {2},
     PAGES = {375--389},
      ISSN = {1661-7207},
   MRCLASS = {20C15 (22F10 37A05)},
  MRNUMBER = {3231220},
MRREVIEWER = {Nhan-Phu Chung},
       DOI = {10.4171/GGD/230},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.4171/GGD/230},
}
	
	
	
\bib{DF}{article}{
  title={On the stabilisers of points in groups with micro-supported actions},
  author={Francoeur, Dominik},
journal = {Journal of Group Theory},
number = {3},
volume = {24},
year = {2021},
pages = {533--547}
  publisher={De Gruyter}
}
	
\bib{G}{article}{
  title={The generation problem in Thompson group $ F$},
  author={Golan, Gili},
  preprint={arXiv:1608.02572},
  year={2016}
}



\bib{G2}{article}{
  title={On Maximal Subgroups of Thompson's Group $F$},
  author={Golan, Gili},
  journal={preprint arXiv:2209.03244},
  year={2022}
}



\bib{GS}{article}{
AUTHOR = {Golan, Gili}, 
    AUTHOR = {Sapir, Mark},    
     TITLE = {On {J}ones' subgroup of {R}. {T}hompson group {$F$}},
   JOURNAL = {J. Algebra},
  FJOURNAL = {Journal of Algebra},
    VOLUME = {470},
      YEAR = {2017},
     PAGES = {122--159},
      ISSN = {0021-8693},
   MRCLASS = {20F65 (20F05 57M25)},
  MRNUMBER = {3565428},
MRREVIEWER = {J. S. Birman},
       DOI = {10.1016/j.jalgebra.2016.09.001},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1016/j.jalgebra.2016.09.001},
}
	
\bib{GS2}{article}{
   AUTHOR = {Golan, Gili}, 
    AUTHOR = {Sapir, Mark},
         TITLE = {On subgroups of {R}. {T}hompson's group {$F$}},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {369},
      YEAR = {2017},
    NUMBER = {12},
     PAGES = {8857--8878},
      ISSN = {0002-9947},
   MRCLASS = {20F65 (20G07)},
  MRNUMBER = {3710646},
MRREVIEWER = {J. S. Birman},
       DOI = {10.1090/tran/6982},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1090/tran/6982},
}

\bib{GS3}{article}{
    AUTHOR = {Golan, Gili}, 
    AUTHOR = {Sapir, Mark},
     TITLE = {On the stabilizers of finite sets of numbers in the {R}.
              {T}hompson group {$F$}},
   JOURNAL = {Algebra i Analiz},
  FJOURNAL = {Rossi\u{\i}skaya Akademiya Nauk. Algebra i Analiz},
    VOLUME = {29},
      YEAR = {2017},
    NUMBER = {1},
     PAGES = {70--110},
      ISSN = {0234-0852},
   MRCLASS = {20F38 (20F05)},
  MRNUMBER = {3660685},
       DOI = {10.1090/spmj/1482},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1090/spmj/1482},
}
		
		
\bib{GS4}{article}{
  title={On closed subgroups of the R. Thompson group $F$},
   AUTHOR = {Golan, Gili}, 
    AUTHOR = {Sapir, Mark},  
    note={preprint \href{http://arxiv.org/abs/2105.00531}{arXiv:2105.00531}},    
 %   journal={preprint arXiv:2105.00531},
  year={2021}
}
	

\bib{GP}{article}{ ,
  title={Conway Rational Tangles and the Thompson Group},
  author={Grymski, Ariana},
  author={Peters, Emily},
  journal={preprint arXiv:2212.00100},
  year={2022}
}

	\bib{HIG}{book}{%higman1974finitely,
  title={Finitely presented infinite simple groups},
  author={Higman, Graham},
  volume={8},
  year={1974},
  publisher={Department of Pure Mathematics, Department of Mathematics, IAS, Australian}
}

		
	\bib{jo2}{article}{
    AUTHOR = {Jones, Vaughan F. R.},
title={Planar Algebras I},
journal={New Zealand Journal of Mathematics},
volume={52},
pages={1-107},
note={preprint \href{http://arxiv.org/abs/9909027}{arXiv:9909027}},
year={2021},
}

		

	\bib{Jo14}{article}{
    AUTHOR = {Jones, Vaughan F. R.},
     TITLE = {Some unitary representations of {T}hompson's groups {$F$} and
              {$T$}},
   JOURNAL = {J. Comb. Algebra},
  FJOURNAL = {Journal of Combinatorial Algebra},
    VOLUME = {1},
      YEAR = {2017},
    NUMBER = {1},
     PAGES = {1--44},
      ISSN = {2415-6302},
   MRCLASS = {57M25 (20F38 46L37 81T40)},
  MRNUMBER = {3589908},
MRREVIEWER = {Conchita Mart\'{\i}nez-P\'{e}rez},
       DOI = {10.4171/JCA/1-1-1},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.4171/JCA/1-1-1},
}





	\bib{Jo16}{article}{
    AUTHOR = {Jones, Vaughan F. R.},
     TITLE = {A no-go theorem for the continuum limit of a periodic quantum
              spin chain},
   JOURNAL = {Comm. Math. Phys.},
  FJOURNAL = {Communications in Mathematical Physics},
    VOLUME = {357},
      YEAR = {2018},
    NUMBER = {1},
     PAGES = {295--317},
      ISSN = {0010-3616},
   MRCLASS = {82B10 (81R12)},
  MRNUMBER = {3764571},
MRREVIEWER = {Lawrence E. Thomas},
       DOI = {10.1007/s00220-017-2945-3},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1007/s00220-017-2945-3},
}

		
 
 
 
 
	\bib{Jo18}{article}{
    AUTHOR = {Jones, Vaughan F. R.},
     TITLE = {On the construction of knots and links from Thompson's       groups},
 BOOKTITLE = {Knots, low-dimensional topology and applications},
    SERIES = {Springer Proc. Math. Stat.},
    VOLUME = {284},
     PAGES = {43--66},
 PUBLISHER = {Springer, Cham},
      YEAR = {2019},
   MRCLASS = {57M25 (20F36 20F38 22D10 57M27)},
  MRNUMBER = {3986040},
       DOI = {10.1007/978-3-030-16031-9\_3},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1007/978-3-030-16031-9_3},
}
		
 
 
 
 
 		
	\bib{Jo19}{incollection}{
    AUTHOR = {Jones, Vaughan F. R.},
title={Irreducibility of the Wysiwyg representations of Thompson's groups},
  booktitle={Representation Theory, Mathematical Physics, and Integrable Systems},
  pages={411--430},
  year={2021},
  publisher={Springer}
}

\bib{Kodama}{article}{%kodama2023p,
  title={The $p$-colorable subgroup of Thompson's group},
  author={Kodama, Yuya and Takano, Akihiro},
  journal={preprint arXiv:2302.10060},
  year={2023}
}


	\bib{Ma}{article}{
    AUTHOR = {Mackey, George W.},
     TITLE = {The theory of unitary group representations},
      NOTE = {Based on notes by James M. G. Fell and David B. Lowdenslager
              of lectures given at the University of Chicago, Chicago, Ill.,
              1955,
              Chicago Lectures in Mathematics},
 PUBLISHER = {University of Chicago Press, Chicago, Ill.-London},
      YEAR = {1976},
     PAGES = {x+372},
   MRCLASS = {22-02},
  MRNUMBER = {0396826},
}

  
 
    	\bib{MPS}{article}{
 AUTHOR = {Morrison, Scott},
 AUTHOR = {Peters, Emily},
 AUTHOR = {Snyder, Noah},
     TITLE = {Categories generated by a trivalent vertex},
   JOURNAL = {Selecta Math. (N.S.)},
  FJOURNAL = {Selecta Mathematica. New Series},
    VOLUME = {23},
      YEAR = {2017},
    NUMBER = {2},
     PAGES = {817--868},
      ISSN = {1022-1824},
   MRCLASS = {18D10 (05C10 57M27)},
  MRNUMBER = {3624901},
MRREVIEWER = {Marko \v{Z}ivkovi\'{c}},
       DOI = {10.1007/s00029-016-0240-3},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1007/s00029-016-0240-3},
}
 
 
     	\bib{NR}{article}{
     AUTHOR = {Nikkel, Jordan},
     AUTHOR = {Ren, Yunxiang},
     TITLE = {On {J}ones' subgroup of {R}. {T}hompson's group {$T$}},
   JOURNAL = {Internat. J. Algebra Comput.},
  FJOURNAL = {International Journal of Algebra and Computation},
    VOLUME = {28},
      YEAR = {2018},
    NUMBER = {5},
     PAGES = {877--903},
      ISSN = {0218-1967},
   MRCLASS = {20F65 (20F05)},
  MRNUMBER = {3844705},
MRREVIEWER = {J\"{o}rg Lehnert},
       DOI = {10.1142/S0218196718500388},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1142/S0218196718500388},
}
		
      	\bib{RS}{article}{
   title={Regular Isotopy Classes of Link Diagrams From Thompson's Groups},
  author={Raghavan, Rushil},
  author={Sweeney, Dennis},
  journal={arXiv preprint arXiv:2008.11052},
  year={2020}
}

      	\bib{Ren}{article}{
    AUTHOR = {Ren, Yunxiang},
     TITLE = {From skein theory to presentations for {T}hompson group},
   JOURNAL = {J. Algebra},
  FJOURNAL = {Journal of Algebra},
    VOLUME = {498},
      YEAR = {2018},
     PAGES = {178--196},
      ISSN = {0021-8693},
   MRCLASS = {43A10 (20F65)},
  MRNUMBER = {3754410},
MRREVIEWER = {M\u{a}d\u{a}lina Roxana Buneci},
       DOI = {10.1016/j.jalgebra.2017.11.018},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1016/j.jalgebra.2017.11.018},
}

	      	\bib{Sav2}{article}{
    AUTHOR = {Savchuk, Dmytro},
     TITLE = {Some graphs related to Thompson's group {$F$}},
 BOOKTITLE = {Combinatorial and geometric group theory},
    SERIES = {Trends Math.},
     PAGES = {279--296},
 PUBLISHER = {Birkh\"{a}user/Springer Basel AG, Basel},
      YEAR = {2010},
   MRCLASS = {20F65},
  MRNUMBER = {2744025},
MRREVIEWER = {Fran\c{c}ois Dahmani},
       DOI = {10.1007/978-3-7643-9911-5\_12},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1007/978-3-7643-9911-5_12},
}
			
	
	      	\bib{Sav}{article}{
     AUTHOR = {Savchuk, Dmytro},
     TITLE = {Schreier graphs of actions of Thompson's group {$F$} on the
              unit interval and on the Cantor set},
   JOURNAL = {Geom. Dedicata},
  FJOURNAL = {Geometriae Dedicata},
    VOLUME = {175},
      YEAR = {2015},
     PAGES = {355--372},
      ISSN = {0046-5755},
   MRCLASS = {20F65 (37C85)},
  MRNUMBER = {3323646},
MRREVIEWER = {Ariadna Fossas},
       DOI = {10.1007/s10711-014-9951-9},
       URL = {https://doi-org.proxy.library.vanderbilt.edu/10.1007/s10711-014-9951-9},
}
	
\bib{Stallings}{article}{ 
  title={Topology of finite graphs},
  author={Stallings, John R.},
  journal={Invent. Math.},
  volume={71},
  number={3},
  pages={551--65},
  year={1983}
}
	

 
\end{biblist}
%\end{bibdiv}
